Performance Improvement of True Time Delay Based Centralized Beamforming Control with the Modulation Instability Phenomenon for Wireless-Array Antennas

This paper proposes a novel method to enhance the performance of the modulator for fifth-generation wireless communication (5G) by exploiting modulation instability (MI). We show that MI can reduce the bias voltage of the modulator ($V_\pi$) by generating carrier side-band gain, and increase the modulation BandWidth (BW), resulting in higher channel capacity, without changing the modulator structure. In receive mode of the array antenna, where the signal is very weak, high-frequency amplification is a high demanding solution to mitigate coverage issue. We also present a developed microwave-photonic beamforming bit-controller system for receiver-transmitter phased array antennas (PAAs), which are essential for high-capacity wireless communications like 5G. We employ a modulated frequency comb exploiting MI fiber to achieve an amplified true-time delay (TTD) technique for wide-coverage PAA beamforming and show that it can steer wideband high-frequency signal to a specific direction angle, avoiding beam-squint.

==> acronym.tex <==
% \acrodef{acronym}[short name]{full name}
\acrodef{IC}[IC]{Integrated Circuit}
% \acrodef{svm}[SVM]{Support Vector Machine}
\newacro{svm}[SVM]{Support Vector Machine}
% Example use \ac{IC} for printing "Integrated Circuit (IC), use \ac{IC} again and it will print (IC)"
% For plural use \acp{IC} for short and \aclp{IC} for long.
% For more see: http://ftp.acc.umu.se/mirror/CTAN/macros/latex/contrib/acronym/acronym.pdf

==> author.tex <==
\author{\IEEEauthorblockN{
Seyed Moien Alavi\IEEEauthorrefmark{1},
Hassan Zakeri\IEEEauthorrefmark{2}, 
Rasoul Azizpour\IEEEauthorrefmark{3}
Gholam Reza Moradi $Senior Member$, $IEEE$, \IEEEauthorrefmark{4}
}

\IEEEauthorblockA{
 Department of Electrical Engineering, Amirkabir University of
Technology, Tehran 15914, Iran\\
Email:
\IEEEauthorrefmark{1}S.M.alavi@aut.ac.ir, 
\IEEEauthorrefmark{2}h.zakeri@aut.ac.ir,
\IEEEauthorrefmark{3}ra.azizpour@aut.ac.ir
\IEEEauthorrefmark{4} ghmoradi aut.ac.ir
}}

==> preamble.tex <==
% Report template for Mälardalen University
% Original template can be found: 
% https://www.overleaf.com/latex/templates/ieee-bare-demo-template-for-conferences/ypypvwjmvtdf
% Template file structure organised by: Emil Persson
% The following packages should follow the IEEE conference guidelines.

% Swedish language package 
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[swedish,english]{babel}

% Graphics
\usepackage{graphicx, float, subfigure, blindtext}

\newcommand\IEEEhyperrefsetup{
bookmarks=true,bookmarksnumbered=true,%
colorlinks=true,linkcolor={black},citecolor={black},urlcolor={black}%
}

% Preferred hyperref setup, Michael Shell
\usepackage[\IEEEhyperrefsetup, pdftex]{hyperref}

% Maths
\usepackage{mathtools}

% These packages must be at the end
\usepackage[nolist,nohyperlinks]{acronym}
\usepackage{cleveref}
\graphicspath{{images/}}
